Experimental Design for Non-Parametric Correction of Misspecified Dynamical Models

We consider a class of misspecified dynamical models where the governing term is only approximately known. Under the assumption that observations of the system's evolution are accessible for various initial conditions, our goal is to infer a non-parametric correction to the misspecified driving term such as to faithfully represent the system dynamics and devise system evolution predictions for unobserved initial conditions. We model the unknown correction term as a Gaussian Process and analyze the problem of efficient experimental design to find an optimal correction term under constraints such as a limited experimental budget. We suggest a novel formulation for experimental design for this Gaussian Process and show that approximately optimal (up to a constant factor) designs may be efficiently derived by utilizing results from the literature on submodular optimization. Our numerical experiments exemplify the effectiveness of these techniques.

==> Emulation.tex <==
\section{Efficient Emulation}\label{sec:emulation}
\color{red}
We apply the mechanism of inference in a GP to derive an estimate for the correction term $\textbf{F}(\cdot)$ based on the observations $\tilde{\textbf{F}}(\mathcal{Y}_m(\mathcal{Y}_0))$. Following the learning stage we use the revised model \eqref{eq:mis_specified_model} to emulate the system output for arbitrary initial conditions. These emulations entail running generic numerical ODE solvers, which require repeated queries $\textbf{F}(\textbf{y})$ for $\textbf{y}\in \mathcal{D}$. With the conventional estimation method \eqref{eq:gaussian_inference} the complexity of each query scales as $O(K')$ which can become prohibitive when the experimental budget is considerable

In lieu of the generic approach we invoke the random feature approximation scheme, as introduced in \cite{rahimi2007random} and apply the explicit regression formulation \eqref{eq:feature_reg_noise} over the proxy feature space. For a Gaussian kernel a finite dimensional feature map $\textbf{z}(\cdot):\mathbb{R}^d\rightarrow\mathbb{R}^D$ may be selected such as to satisfy
\begin{align}
	k(\textbf{y}_1,\textbf{y}_2)=\langle \boldsymbol\phi(\textbf{y}_1), \boldsymbol\phi(\textbf{y}_2) \rangle\approx 
	\langle \textbf{z}(\textbf{y}_1), \textbf{z}(\textbf{y}_2) \rangle
\end{align}
Substituting $\textbf{z}(\textbf{y})$ for $\boldsymbol\phi(\textbf{y})$, an approximate explicit representation for $ \textbf{F}(\textbf{y})$ in terms of the features $\textbf{z}(\textbf{y})$ holds according to $\textbf{F}(\textbf{y})\approx\hat{\boldsymbol{\Theta}}_l^T \textbf{z}(\textbf{y})$.

Specifically, one choice for $\textbf{z}(\textbf{y})$ that satisfies the above approximation is taking $\textbf{z}(\textbf{y})=\cos(\textbf{W}\textbf{y}+\textbf{b})$ where $\textbf{W}$ is a random matrix with independent rows distributed according to $\textbf{w}_{i}\sim \mathcal{N}(0,\frac{1}{\sigma^{2}}I)$ and $\textbf{b}$ a random vector drawn uniformly as $b_i\sim U[0,2\pi]$.

The computational complexity of each query in this formulation scales as $O(D)$ instead of $O(\tilde{K})$ which may be substantial. (Here can quote Theorem about required $D$ for high fidelity representation.
\color{black}

